Thermodynamically Driven Signal Amplification

The field of chemical computation attempts to model computational behavior that arises when molecules, typically nucleic acids, are mixed together. Thermodynamic binding networks (TBNs) is a highly abstracted model that focuses on which molecules are bound to each other in a "thermodynamically stable" sense. Stability is measured based only on how many bonds are formed and how many total complexes are in a configuration, without focusing on how molecules are binding or how they became bound. We study the problem of signal amplification: detecting a small quantity of some molecule and amplifying its signal to something more easily detectable. This problem has natural applications such as disease diagnosis. By focusing on thermodynamically favored outcomes, we seek to design chemical systems that perform the task of signal amplification robustly without relying on kinetic pathways that can be error prone and require highly controlled conditions (e.g., PCR amplification). It might appear that a small change in concentrations can result in only small changes to the thermodynamic equilibrium of a molecular system. However, we show that it is possible to design a TBN that can "exponentially amplify" a signal represented by a single copy of a monomer called the analyte: this TBN has exactly one stable state before adding the analyte and exactly one stable state afterward, and those two states "look very different" from each other. We also show a corresponding negative result: a doubly exponential upper bound, meaning that there is no TBN that can amplify a signal by an amount more than doubly exponential in the number and sizes of different molecules that comprise it. Our work informs the fundamental question of how a thermodynamic equilibrium can change as a result of a small change to the system (adding a single molecule copy).

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> old_fragments.tex <==

% \begin{defn}
%     Given configurations $\alpha$ and $\beta$ in a TBN, we say $\alpha \splitsto^1 \beta$ (equivalently, $\beta \mergesto^1 \alpha)$ if there are two polymers in $\beta$ such that $\alpha$ is the configuration obtained from $\beta$ by replacing those two polymers with their union.
% \end{defn}




% \begin{defn}[(Hausdorff) distance between sets of configurations]
% Let $\mathcal C$ and $\mathcal C'$ be sets of configurations in some TBNs. The \emph{asymmetrical} distance $d^*(\mathcal C, \mathcal C')$ is given by:
% \[d^*(\mathcal C,\mathcal C') = \max_{\alpha \in \mathcal C} \min_{\beta \in \mathcal C'} d(\alpha, \beta).\]
% That is, it is given by choosing a single configuration from $\mathcal C$ that is the farthest away from its closest configuration from $\mathcal C'$. The symmetrical distance $d(\mathcal C, \mathcal C')$ is defined by
% \[d(\mathcal C, \mathcal C') = \max \{d^*(\mathcal C, \mathcal C'), d^*(\mathcal C', \mathcal C)\}\]
% \end{defn}

% \begin{defn}[distance between TBNs]
% Given TBNs $T$ and $T'$, let $\mathcal C$ and $\mathcal C'$ be their stable configurations. Define the distance between $T$ and $T'$ as 
% \[d(T, T') = d(\mathcal C, \mathcal C').\]
% Let $\mathcal C_k$ and $\mathcal C_k'$ be the sets of saturated configurations in $T$ and $T'$ respectively whose distance to stability is at most $k$. Then define the $k$-distance between $T$ and $T'$ as
% \[d_k(T, T') = d(\mathcal C_k, \mathcal C_k').\]
% \end{defn}
% To say that $d_k(T, T') = n$ is to say that we can distinguish between $T$ and $T'$ with signal strength proportional to $n$ and reliability proportional to $k$.

% \begin{defn}[distance between sets of configurations]
% Let $\mathcal C$ and $\mathcal C'$ be sets of configurations in some TBNs. Then we define the distance between these sets as:
% \[d^*(\mathcal C,\mathcal C') = \min_{\alpha \in \mathcal C, \beta \in \mathcal C'} d(\alpha, \beta).\]
% \end{defn}

% \begin{defn}[distance between TBNs]
% Given TBNs $T$ and $T'$, let $\mathcal C$ and $\mathcal C'$ be their stable configurations. Define the distance between $T$ and $T'$ as 
% \[d(T, T') = d(\mathcal C, \mathcal C').\]
% Let $\mathcal C_k$ and $\mathcal C_k'$ be the sets of saturated configurations in $T$ and $T'$ respectively whose distance to stability is at most $k$. Then define the $k$-distance between $T$ and $T'$ as
% \[d_k(T, T') = d(\mathcal C_k, \mathcal C_k').\]
% \end{defn}
% To say that $d_k(T, T') = n$ is to say that we can distinguish between $T$ and $T'$ with signal strength proportional to $n$ and reliability proportional to $k$.

% \begin{defn}
% If a TBN $T$ is a detector for $A$, then we say $T$ has \emph{entropy gap} $k$ if any saturated, locally stable configuration of $T$ in which at least one $F$ monomer is in a polymer with no $Q$ monomers has distance to stability at least $k$ (that is, it has at least $k$ fewer polymers than any stable configuration). 
% \end{defn}

% \begin{thm}For any integers $n \geq 1, k \geq 2$, there exists a TBN $T_{n,k}$ and monomer $A$ such that $G$ is a detector for $A$ with strength $2^{n-1}$ and entropy gap $k - 1$. \end{thm}



% Define the TBN $T_{n,k}$ as follows: it has monomer types $\mathbf{U}_{i,j}$ and $\mathbf{S}_{i,j}$ (those with only unstarred sites, and those with both starred and unstarred sites) for $1\leq i \leq n, 1 \leq j \leq k$. It also has monomer types $\mathbf{G}_i$ and $\mathbf{G}_i^*$ (full grid gates) for each $2 \leq i \leq n$. It has domain types $(i,j,\ell)$ for $1 \leq i \leq n + 1, 1 \leq j, \ell \leq k$. Each monomer $\mathbf{U}_{i,j}$ has $k$ different unstarred domains, one of each $(i,j,\ell)$ for each $1 \leq \ell \leq k$. Each monomer $\mathbf{S}_{i,j}$ has a starred copy of each domain in $\mathbf{U}_{i,j}$, and additionally has two copies of each unstarred domain $a_{i+1,\ell,j}$ for each $1 \leq \ell \leq k$ (note that here the second domain type parameter varies instead of the third). Each $\mathbf{G}_i$ consists of one copy of each unstarred domain $(i,j,\ell)$ for each $1 \leq j, \ell \leq k$. Each $\mathbf{G}_i^*$ consists of the same domains but all starred. For each monomer type $\mathbf{U}_{i,j}, \mathbf{S}_{i,j}, \mathbf{G}_i$ and $\mathbf{G}_i^*$, there are $2^{i-1}$ copies of that monomer type. The set $F$ contains all $\mathbf{S}_{n,j}$ and the set $Q$ contains all $\mathbf{U}_{n,j}$ (notably, this means it will have strength $2^{n-1}$ as a detector). The analyte $\mathbf{A}$ is a monomer that looks like what $\mathbf{G}_1$ would if $T_{n,k}$ contained it: it has one copy of each unstarred domain $a_{1,j,\ell}$. 


% \begin{defn}
% Given a TBN $T$, let $G(T)$ be a directed graph in which the vertices are given by monomers in $T$ and for each site type, edges are drawn from all monomers with that unstarred site to all monomers with the matching starred site. We say that $T$ is \emph{feed-forward} if $G$ is acyclic.
% \end{defn}



% \begin{lem}
% Given a stable configuration $C$ of a TBN $T$, it is always possible to order the merges that bring the all-separated configuration to $C$ in such a way that, if carried out in that order, every merge covers at least one starred site.
% \end{lem}

% \begin{proof}
% Starting from all monomers being separated, we simply repeatedly choose any merge from $C$ that directly covers at least one starred site. There will always be at least one choice of such a merge until we reach $C$, as there will always be at least one uncovered starred site; if there were a configuration that we reached before $C$ with all starred sites covered, then $C$ would not be stable. 
% \end{proof}

% We call such an ordering of merges a \emph{canonical ordering}. 



% After each merge, we can keep track of the total number of polymers with at least one uncovered starred site. The only way that this count could ever go down by more than one is by merging two polymers with uncovered starred sites to obtain a polymer without any uncovered starred sites. This cannot happen with our given merge ordering: each time that we merge a polymer $P_1$ from $C$ on to some polymer $P_2$ that we've created by merging polymers from $C$, because $P_1$ occurs at least as late in $L$ as any other polymer already in $P_2$, we see that $P_1$ cannot cover any uncovered starred sites on any monomers already in $P_2$. It follows that either $P_2$ has no uncovered starred sites, or merging $P_1$ into $P_2$ will create a polymer that has uncovered starred sites. In either case, the count of polymers with uncovered starred sites cannot decrease by more than one from any merge. It follows that since the initial value of this count is equal to the number of polymers with at least one uncovered starred site, and the value of this count in $S$ must be zero, this value serves as a lower bound on the number of merges that must be performed to get to a stable configuration.


% \begin{proof}
% Given a feed-forward TBN $T$ starting from a configuration with all monomers separated, to get to some stable configuration $C$ we may carry out a canonically-ordered series of merges. We may simultaneously carry out the same series of merges of vertices in $G(T)$: when we merge two vertices, we obtain a new vertex representing a new polymer, and we maintain any edges that were not between the two merged vertices. At each step, we keep track of the number of polymers with at least one uncovered starred site. If any single merge ever reduces this count by two, it must be the case that two polymers with uncovered starred sites were merged together to form a single polymer with no uncovered starred sites. This implies that both polymers had unstarred sites that the other 
% \end{proof}


% \begin{proof}We observe that $\widetilde{T}_{n,k}$ is feed-forward by ordering its monomers first by increasing value of layer, and then for each layer $i$ in the order $\mathbf{G}_i$, then all of the $\mathbf{U}_{i,j}$, then $\mathbf{G}_i^*$, then all of the $\mathbf{S}_{i,j}$. There is exactly one way to cover all starred sites by making merges equal to $\starriness(\melt(T))$: each $\mathbf{G}_i^*$ can only be covered fully by a $\mathbf{G}_i$, and then each $\mathbf{S}_{i,j}$ can only be covered fully by a $\mathbf{U}_{i,j}$. Thus, by By \cref{cor:stable-if-requires-exactly-s-merges}, this configuration $\widetilde{\sigma}_{n,k}$ is stable, and because no other saturated configuration has this few merges, it is uniquely stable.\end{proof}

% Let $\widetilde{T}'_{n,k}$ be $\widetilde{T}_{n,k}$ with one copy of $\mathbf{A}$ added. We now show that this adding $\mathbf{A}$ have a large effect on stable configurations.

% \begin{lem}
% $\widetilde{T}'_{n,k}$ has a stable configuration $\widetilde{\sigma}_{n,k}^*$ in which no copies of $\mathbf{S}_{n,j}$ are in polymers with any copies of $\mathbf{U}_{n,j}$.
% \end{lem}



% \begin{proof}As $\mathbf{A}$ has no starred sites, the same argument shows that $\widetilde{\sigma}_{n,k}$, together with the free copy of $\mathbf{A}$, is stable (we can put $\mathbf{A}$ at the beginning of our feed-forward ordering). From this stable configuration, we can make a series of an equal number of merges and splits to obtain a configuration with the desired property as follows: split each of the $k$ $\{\mathbf{S}_{1,j}, \mathbf{U}_{1,j}\}$ polymers, and then merge all $k$ of the $\mathbf{S}_{1,j}$ to $\mathbf{A}$. This polymer containing $\mathbf{A}$ will then have two copies of each unstarred site from layer 2 (that is, each unstarred site $(2, j, \ell)$. This means that now, we can split all $2k$ of the $\{\mathbf{S}_{2,j}, \mathbf{U}_{2,j}\}$ polymers and merge all of the $\{\mathbf{S}_{2,j}$ to this polymer containing $\mathbf{A}$. We can continue in this fashion for each $i$ sequentially from $1$ to $n$, at each step making $k\cdot 2^{i-1}$ splits of $\{\mathbf{S}_{i,j}, \mathbf{U}_{i,j}\}$ pairs, followed by $k \cdot 2^{i-1}$ merges to merge all of the $\mathbf{S}_{i,j}$ to the polymer containing $\mathbf{A}$. 

% At each step, the same number of splits and merges are performed and all starred sites end up covered, so the resulting configuration is stable. The last step will split all $\{\mathbf{S}_{n,j}, \mathbf{U}_{n,j}\}$ polymers, of which there are at least $2^n$, implying that $d(\widetilde{\sigma}_{n,k}, \widetilde{\sigma}_{n,k}^*) \geq 2^n$.\end{proof}
% % It follows from these two lemmas that $\widetilde{T}_{n,k}$ is a detector for $A$.\\\\
% % \begin{proof}[Proof of theorem 1.4] The last step to show is that $\widetilde{T}_{n,k}$ has entropy gap $k - 1$. We will show the stronger statement that any saturated, locally stable configuration of $\widetilde{T}_{n,k}$ \emph{at all} other than $\widetilde{\sigma}_{n,k}$ has distance to stability at least $k - 1$.\\\\

% We now demonstrate that this sequence of merges and splits is very unlikely to happen in the absence of the analyte:

% \begin{lem}
%     $\widetilde{T}_{n,k}$ has an entropy gap of $k - 1$. 
% \end{lem}

% \begin{proof}
% As $\widetilde{\sigma}_{n,k}$ is the only stable configuration, we must show that any other saturated configuration of $\widetilde{T}_{n,k}$ can either be split to reach $\widetilde{\sigma}_{n,k}$ (that is, it is $\widetilde{\sigma}_{n,k}$ with some additional merges), or has distance to stability at least $k - 1$. To this end, let $\alpha$ be some saturated configuration of $\widetilde{T}_{n,k}$ with $\alpha \not\splitsto \widetilde{\sigma}_{n,k}$. We must show that $\alpha$ has distance to stability at least $k - 1$, or equivalently, that its merginess is at least $k - 1$ more than that of $\widetilde{\sigma}_{n,k}$.

% If every polymer contains an equal number of $\mathbf{S}_{i,j}$ and $\mathbf{U}_{i,j}$ for all $i, j$, then $\alpha \splitsto \widetilde{\sigma}_{n,k}$. Therefore, there is some $i, j$ such that some polymer contains more $\mathbf{S}_{i,j}$ than $\mathbf{U}_{i,j}$. Since $\alpha$ is saturated, the starred sites on this extra $\mathbf{S}_{i,j}$ must be covered by something other than sites on $\mathbf{U}_{i,j}$ monomers, and the only other monomers that can cover it are $\mathbf{S}_{i-1,\ell}$ monomers. In particular, this polymer must contain one copy of each $\mathbf{S}_{i-1,\ell}$ for each $1 \leq \ell \leq k$. Let $\mathbf{M}$ be one of these $\mathbf{S}_{i,j}$ monomers.

% In order to get from $\melt(\widetilde{T}_{n,k})$ to $\alpha$, we must merge $\mathbf{M}$ to these $k$ other monomers that jointly cover it. Consider then the configuration $\beta$ in which only these $k$ merges have been done. We will show that to get from $\beta$ to $\alpha$ takes at least $\merginess(\widetilde{\sigma}_{n,k}) - 1$ additional merges (noting that $\merginess(\widetilde{\sigma}_{n,k})$ is the number of merges from $\melt(\widetilde{T}_{n,k})$ to the stable $\widetilde{\sigma}_{n,k}$), which implies that $\merginess(\alpha)$ is at least $\merginess(\widetilde{\sigma}_{n,k}) + (k - 1)$. This in turn will show that $\alpha$ has the desired high distance to stability.

% There are $\starriness(\melt(\widetilde{T}_{n,k})) = \merginess(\widetilde{\sigma}_{n,k})$ total monomers with starred sites and only $\mathbf{M}$ can have its starred sites covered in $\beta$, by examination. So $\beta$ contains $\merginess(\widetilde{\sigma}_{n,k}) - 1$ monomers with starred sites that still need to be covered. Note that this is not the value of $s(\beta)$, as some of these starred sites  have been brought together into the same polymer. We know that the starred domain types on $\mathbf{M}$ are $(i,j,\ell)^*$ for $1 \leq \ell \leq k$. Our strategy is to carry out the remaining merges to get from $\beta$ to $\alpha$ in the following order: first, we perform any inclusion-minimal set of merges necessary to reach a configuration where all $(i-1,\ell_1,\ell_2)^*$ sites, $1 \leq \ell_1, \ell_2 \leq k$, are covered. Then we do the same for $((i-2),\ell_1,\ell_2)^*$ sites, and so on until we've covered everything up to and including all $(1,\ell_1,\ell_2)^*$ sites. Lastly we will perform all remaining merges for all $(i,\ell_1,\ell_2)^*$ sites with $i \geq x$ in one step. Our goal at each step is to account for merges in such a way to show that there must be at least one merge for each monomer with starred sites other than $\mathbf{M}$.

% In $\beta$, the only merges thus far carried out will have been to merge one copy of each $\mathbf{S}_{i-1,\ell}$ on to $\mathbf{M}$, to form a polymer $P$. This means that the only thing that will have been done to any $(i-1,\ell_1,\ell_2)$ sites is that some starred sites may have been brought together, but all such unstarred sites will still be on separate monomers. Additionally, $P$ does not have any duplicate $(i-1, \ell_1, \ell_2)^*$ sites, because the monomers that cover $M$ all have distinct sites. We can now establish a lower bound on the number of merges needed to cover all of these starred sites in our first step based only on the number of starred sites we must cover. The only monomers with these unstarred sites are $\mathbf{U}_{i-1, \ell}$ and $\mathbf{S}_{i-2, \ell}$ monomers, each of which has a total of $k$ distinct unstarred $(i-1, \ell_2, \ell_2)$ sites. Therefore, to cover the $k^2$ distinct starred sites at this layer on $P$, it will require at least $k$ merges, that is, one merge for each monomer in $P$ that has these starred sites. 

% In fact, it will require merging either one copy of each $\mathbf{U}_{i-1, \ell}$ or one copy of each $\mathbf{S}_{i-2, \ell}$, because the starred sites we need to cover effectively form a $k \times k$ grid, and the $\mathbf{U}_{i-1, \ell}$ cover this grid by rows and the $\mathbf{S}_{i-2, \ell}$ cover it by columns. In order to cover the whole grid, we need either all the rows or all the columns.

% It follows that the whole process of merges to cover all $(i-1, \ell_1, \ell_2)^*$ sites must make at least one merge per monomer with these sites, as all other such monomers not in $P$ must also each be merged to something.

% \todoi{I had to rewrite part of this to ensure no duplicate starred sites are brought together, which I realized was an oversight of the previous writeup, because S monomers have multiple copies of unstarred sites. Double check that this makes sense.}
% Because we choose the merges in this step to be inclusion-minimal, doing this process for the $(i-1, \ell_1, \ell_2)^*$ sites cannot bring together any $(i-2,\ell_1,\ell_2)$ unstarred sites, only possibly some starred sites. This is because no monomers that have $(i-2,\ell_1,\ell_2)$ unstarred sites have any starred or unstarred $(i-1,\ell_1,\ell_2)$ sites, so no merges involving them could possibly be necessary to cover all $(i-1,\ell_1,\ell_2)^*$ sites. Additionally, it cannot bring together any duplicate $(i-2, \ell_1, \ell_2)^*$ sites: this is because covering the sites in $P$ required us to either cover its $k \times k$ grid of starred sites horizontally or vertically, and either way, none of the monomers used to cover it use duplicate starred sites (and the sequence of merges is inclusion-minimal, so we cannot use both horizontal and vertical monomers to cover it). Covering the other $\mathbf{S}_{i-1, \ell}$ monomers also cannot bring together duplicate starred sites, as the only inclusion-minimal ways to cover them are to either use a single $\mathbf{U}_{i-1, \ell}$ or to use one copy of each $\mathbf{S}_{i-2, \ell}$. 

% Since no unstarred sites and no duplicate starred sites are brought together, the same logic we used for $(i-1,\ell_1,\ell_2)$ sites applies for the $(i-2,\ell_1,\ell_2)$ sites. It follows inductively that doing all of the merges required to cover \emph{all} starred sites from layers before $M$ from the configuration $\beta$ will require at least one merge per monomer with one of these starred sites.

% % The total number of $(x-1,j,\ell)^*$ sites across all monomers is $2k^22^{x-2}$, half from $\mathbf{G}_x^*$ monomers and half from $\mathbf{S}_{x,j}$ monomers. Because no monomers with unstarred $(x-1,j,\ell)$ sites have been brought together yet, even using all $\mathbf{G}_x$ monomers (which have the most of these unstarred sites), merging in enough unstarred sites to cover all of these starred sites would require merging all of the $\mathbf{G}_x$ monomers along with at least $k\cdot 2^{x-2}$ copies of $\mathbf{U}_{x-1,j}$ and/or $\mathbf{S}_{x-2,j}$ monomers. This is exactly equal to the number of monomers with at least one $(x-1,j,\ell)^*$ site on them.
% % Therefore, in order to cover all $(x-1,j,\ell)^*$ sites we must merge in that many (free) monomers, and we may order these merges to always merge these free monomers on to polymers with starred sites that they cover, showing that this also gives a lower bound on the total number of merges required to cover all these starred sites. 
% Now, from this new configuration, we must still make more merges to cover all of $(x,\ell_1,\ell_2)^*$ sites with $x \geq i$. But all of the merges we've made in the previous steps must cover a starred site with a lower first index than $i$, meaning they must have only merged together monomers containing at least one starred or unstarred site with first index at most $i - 1$. None of these monomers contain any \emph{starred} sites with first index at least $i$ (with the exception of $\mathbf{M}$, whose sites are already covered), so it follows that all of these starred sites are all on different monomers. This intermediate configuration is also feed-forward: we can make an ordering as follows. Start with all polymers that have been created from previous steps (whose starred sites must all be covered). No other merges can have been made, since monomers with starred sites $(x,\ell_1,\ell_2)$ with $x \geq i$ cannot have any unstarred sites $(x,\ell_1,\ell_2)$ with $x < i$, so we may take the rest of our ordering of free monomers in the order they are in $\widetilde{T}_{n,k}$'s feed-forward ordering. Since this configuration is feed-forward, by \cref{lem:one-merge-per-monomer} at least one merge per such monomer must be made to get from this configuration to a saturated one.

% Accounting for all of this, from $\beta$, we see that ordering the merges necessary to get to a saturated configuration in this way requires that we have at least one merge per monomer with any starred sites whose first index is either less than $i$, or greater than or equal to $i$, with the exception of the monomer $\mathbf{M}$. As there are $\starriness(\melt(\widetilde{T}_{n,k})) = \merginess(\widetilde{\sigma}_{n,k})$ such monomers including $\mathbf{M}$, we must make $\merginess(\widetilde{\sigma}_{n,k}) - 1$ total merges, showing that the configuration $\alpha$ must have a distance to stability of at least $k - 1$ as desired.

% % Let $C$ be some saturated, locally stable configuration of $\widetilde{T}_{n,k}$ other than $\widetilde{\sigma}_{n,k}$. Let $m$ be the number of merges to get from a configuration of all singletons to $\widetilde{\sigma}_{n,k}$ (that is, the optimal number of merges). If every $\mathbf{S}_{i,j}$ monomer is paired with a $\mathbf{U}_{i,j}$ monomer and every $\mathbf{G}_i^*$ is paired with a $\mathbf{G}_i$, then we can split until we reach $\widetilde{\sigma}_{n,k}$, meaning $C$ wouldn't be locally stable. So some monomer containing starred sites must be in a polymer without the monomer that covers it in the stable configuration. If this monomer is a $\mathbf{S}_{i,j}$ that is covered by a $\mathbf{G}_i$, then there must also be at least one $\mathbf{G}_i^*$ that is not covered by a $\mathbf{G}_i$. It follows that no matter what, there must be some monomer $M$ with starred domains that is bound to at least $k$ other monomers; this is because the only monomers that can cover more than a single one out of $k$ starred domain from $\mathbf{S}_{i,j}$ are $\mathbf{U}_{i,j}$ and $\mathbf{G}_i$, and the only monomer that can cover more than $k$ of the $k^2$ starred domains in $\mathbf{G}_i^*$ is $\mathbf{G}_i$. Consider then the configuration $C'$ in which only these $k$ merges have been done to form a new polymer $P$. We can see that $C'$ is a feed-forward configuration: we see this because we can take the ordering of monomers from $\widetilde{T}_{n,k}$, remove the monomers that have been merged to form $P$, and then insert $P$ at the spot where the earliest one of these removed monomers was. All of the starred sites from $M$ are covered, so the only possible uncovered starred sites in $P$ come from the monomers covering $M$, and those starred sites will never be moved to a part of the ordering before the corresponding unstarred sites. It follows that since $C'$ is feed-forward, by lemma 1.6, 



% % We will show that to get from $C'$ to $C$ takes at least $m - 1$ additional merges, which implies that to get to $C$ from the all-singleton state requires $m + (k - 1)$ merges. \\\\
% % Because there are $m$ total monomers with starred sites and only $M$ is covered in $C'$, it contains $m - 1$ monomers with starred sites that still need to be covered. Suppose that $M$ is a monomer whose starred domain types are $a_{x,j,\ell}$ for some particular value $x$. Then we can carry out the remaining merges to get from $C'$ to $C$ in the following order: first, we carry out all merges that cover at least one $a_{x-1,j,\ell}^*$ site; then all that cover at least one $a_{{x-2},j,\ell}^*$ site, and so on until we've covered everything up to all $a_{1,j,\ell}^*$ sites. Lastly we will carry out the remaining merges for all $(i,j,\ell)^*$ sites with $i \geq x$.\\\\
% % In $C'$, the only merges thus far carried out will have been to merge some copies of $\mathbf{U}_{x,j}$ and/or $\mathbf{S}_{x-1,j}$ on to $M$ (because we know $M$ requires all $k$ or more monomers merged to it to cover it, and these are the only monomers that can possibly cover part of $M$ without covering it completely). This means that the only thing that will have been done to any $a_{x-1,j,\ell}$ sites is that some starred sites may have been brought together, but all unstarred $a_{x-1,j,\ell}$ sites will still be on separate monomers. The total number of $a_{x-1,j,\ell}^*$ sites across all monomers is $2k^22^{x-2}$, half from $\mathbf{G}_x^*$ monomers and half from $\mathbf{S}_{x,j}$ monomers. Because no monomers with unstarred $a_{x-1,j,\ell}$ sites have been brought together yet, even using all $\mathbf{G}_x$ monomers (which have the most of these unstarred sites), merging in enough unstarred sites to cover all of these starred sites would require merging all of the $\mathbf{G}_x$ monomers together with at least $k\cdot 2^{x-2}$ copies of $\mathbf{U}_{x-1,j}$ and/or $\mathbf{S}_{x-2,j}$ monomers. This is exactly equal to the number of monomers with at least one $a_{x-1,j,\ell}^*$ site on them. Doing this process does not bring together any $a_{x-2,j,\ell}$ unstarred sites, so it follows inductively that doing all of the merges required to cover \emph{all} $(i,j,\ell)^*$ sites with $i < x$ from the configuration $C'$ will require at least one merge per monomer with one of these starred sites.\\\\
% % Now, from this new configuration, we must still make more merges to cover all of $(i,j,\ell)^*$ sites with $i \geq x$. But all of the merges we've made in the previous step must cover a starred site with a lower first index than $x$, meaning they must have only merged together monomers containing at least one starred or unstarred site with first index at most $x - 1$. None of these monomers contain any \emph{starred} sites with first index at least $x$ (with the exception of $M$, whose sites are already covered), so it follows that all of these starred sites are all on different monomers, so necessarily at least one merge per such monomer must be made to get from this configuration to a saturated one.\\\\
% % Accounting for all of this, from $C'$, we see that ordering the merges necessary to get to a saturated configuration in this way requires that we have at least one merge per monomer with any starred sites whose first index is either less than $x$, or greater than or equal to $x$, with the exception of the monomer $M$. As there are $m$ such monomers including $M$, we must make $m - 1$ total merges, showing that the configuration $C$ must have a distance to stability of at least $k - 1$ as desired.
% \end{proof}


% The following is a useful lemma applicable more broadly to TBNs that can give some intuition for what these new monomers will do:

% \begin{lem}
%     \label{lem:complement}
%     Suppose a TBN $T$ has an entropy gap of $k$. Suppose a new TBN $T'$ is formed by adding some monomers $\mathbf{M}_1, \mathbf{M}_2, \ldots, \mathbf{M}_m$, with $2 \leq m \leq k + 1$, that are perfectly complementary: that is, the polymer $P = \{\mathbf{M}_i : 1 \leq i \leq m\}$ has no unbound sites. Then:
%     \begin{enumerate}
%         \item There is a stable configuration of $T'$ in which $P$ appears as a polymer.
%         \item $T'$ has an entropy gap of $k - (m - 2)$.
%     \end{enumerate} 
% \end{lem}

% For example, recall that all TBNs have an entropy gap of 1 trivially. Thus, when $m = 2$, this lemma says that when adding two perfectly complementary monomers (such as $\mathbf{G}$ and $\mathbf{G}^*$), it is always possible to put them together in a stable configuration. We need this slight generalization to more easily reason about $\mathbf{H}$ and $\mathbf{H}^*$. 

% In some sense, this lemma is a companion to the main theorem of this paper: it says that it is impossible to drastically change the stable configurations of a TBN by adding a set of \emph{mutually complementary} monomers. 

% \begin{proof}
%     Let $\alpha$ be any stable configuration of $T$. If we simply add $P$ to $\alpha$, we get a saturated configuration of $T'$ that has distance to stability 
    
    
%     Let $\alpha'$ be any stable configuration of $T'$. If all the $\mathbf{M}_i$ are together in a polymer in $\alpha'$, then because $P$ has no unbound sites, there cannot be any other monomers together with them as they would be able to collectively split off to increase the number of polymers without breaking any bonds.

%     Otherwise, each $\mathbf{M}_i$ is in a (not necessarily distinct) polymer $P_i$, $1 \leq i \leq m$. Suppose there are $n \leq m$ such distinct polymers. Note that because this is a stable configuration, these polymers must be self-saturated. In this case, suppose we take $\alpha'$, join all of these $P_i$ together, and then split off all the $M_i$ from the resulting polymer to form $P$. Then we take the resulting polymer from which we removed $P$, and, if it can be split without uncovering any starred sites, we split it in such a way until it can't. The result of this must be a saturated configuration: this is because we start with a saturated configuration, merge some polymers together, split off an equal number of starred and unstarred sites (because the $\mathbf{M}_i$ are perfectly complementary), and then possibly make some extra splits that don't uncover any starred sites. 
    
%     If we then remove $P$, we get a saturated configuration of $T$. This configuration cannot split to any other saturated configuration: all of the polymers in it either came from the process just described (in which we made as many splits as possible without uncovering any starred sites), or they came from the stable configuration $\alpha'$. Therefore, because $T$ has an entropy gap of $k$, this resulting configuration must either be stable, or be distance at least $k$ from stability. It follows that if we re-add $P$ to the configuration, we get a configuration of $T'$ that 
    
%     remove these two polymers, and add polymers $\{M, M^*\}$ and $A \cup B$. We must show that the polymer $A \cup B$ is self-saturated. if it had an unbound starred site on a monomer in $A$, then that starred site must be covered by $M$ in the polymer $M \cup A$, because it is self-saturated. Thus, since that unstarred site appears in $M$, the corresponding starred site must exist on $M^*$, meaning that it is covered by some monomer in $B$ in the polymer $M^* \cup B$, because it is also self-saturated. Thus, starred sites on monomers in $A$ are covered by monomers in $B$, and vice versa. \todo{Make sure I define self-saturated} Thus, this new configuration has the same number of polymers, and all its polymers are self-saturated, so it is stable.
% \end{proof}

% \begin{cor}
%     Let $T$ be a TBN with stable configuration $\alpha$. Let $T'$ be $T$ with one extra copy each of two perfectly complementary monomers $M$ and $M^*$. Then $\alpha + \{M, M^*\}$ is a stable configuration of $T'$.
% \end{cor}

% \begin{proof}
%     By \cref{lem:complement}, some stable configuration of $T'$ contains $\{M, M^*\}$; choosing how to partition the rest of the monomers of $T'$ in such a configuration is equivalent to choosing a stable configuration of $T$, so we may choose $\alpha$.
% \end{proof}



% \todoi{I might be able to remove everything that talks about Gomory functions, from here on}
% \subsection{Gomory Functions}

% This sensitivity analysis problem was studied by Blair and Jeroslow in \cite{blair1982ip}. They show that the optimal value of an IP is given by a Gomory function of the right-hand side: a function built up from its inputs by taking positive linear combinations, ceiling functions, and maxima. The proof they give is constructive, so it can be used to construct a bound on the coefficients of these linear combinations, which can in turn be used to bound the difference in the objective function (i.e., the optimal number of polymers) after adding one copy of a monomer. They also use this result to show that for any IP problem there is some set of "unrestricted" Gomory functions (in which negative linear combinations are also allowed), which, when given the right-hand side of that IP, produce variable values for some optimal solution. This isn't quite sufficient for our purposes, as it only shows that \emph{some} configuration before and after adding a monomer must be close. To correspond with the notion of Hausdorff distance, we must show that, given \emph{any} configuration in one TBN, we can find a "close" configuration to it in the other (and vice versa). We do this using a similar technique to theirs. As we don't care about the distinction between regular and unrestricted Gomory functions, we simply use the latter as our definition. 

% \begin{defn}
%     A function $f: \mathbb Z^n \to \mathbb Z$ is an (unrestricted) \emph{Gomory function} if it can be written as a finite nested application of the following operations on its inputs:
%     \begin{enumerate}
%         \item Rational linear combinations
%         \item The ceiling function $\lceil x \rceil$ giving the least integer greater than or equal to $x$
%         \item Maxima
%     \end{enumerate}
% \end{defn}

% Proposition 2.18 from Blair and Jeroslow tells us that Gomory functions can always be written as a single maximum of finitely many Chv\'atal functions, which are Gomory functions without maxima. While their proof is about "restricted" Gomory functions, it works for unrestricted ones as well. This allows the following definition:
% \todoi{Leaving this in for now, but I think the standard form stuff may be unneeded}

% \begin{defn}
%     A Gomory function is written in \emph{standard form} if it contains only a single maximum at the outermost layer of nesting.
% \end{defn}

% Blair and Jeroslow show that Gomory functions have a rank, which is essentially the number of nesting operations needed to define it. Informally, a Gomory function of a given pre-rank can be written by using one of the three given operations on Gomory functions of lower pre-ranks, and a Gomory function's rank is its least pre-rank. 

% We need some way to bound how quickly the output of a Gomory function changes.

% \begin{defn}
%      We say that a Gomory function has \emph{bounded slope} by some bound $m$ if it can be written in standard form such that for any nested sequence of operations, the product of all coefficients appearing in rational linear combinations in that sequence is at most $m$.
% \end{defn}

% \begin{lem}
%     \label{lem:slopebound}
%     Let $f: \mathbb Z^n \to \mathbb Z$ be a Gomory function with slope bound $m$ and rank $r$. Then given $x, y \in \mathbb Z^n$, if $\left|\left|x - y\right|\right|_1 \leq 1$, then $\left|f(x) - f(y)\right| \leq m + 2r$.
% \end{lem}

% \begin{proof}
%     We proceed by induction on rank. If $f$ is linear, its slope bound is its slope and the result is immediate. 

%     If $f = \lceil g \rceil$ where $g$ is of lower rank than $f$, then $g$ must have the same slope bound as $f$ so by the inductive hypothesis $g(x) - g(y) \leq m + (2r - 2)$, and $|f - g| \leq 1$, so by the triangle inequality $|f(x) - f(y)| \leq |f(x) - g(x)| + |g(x) - g(y)| + |g(y) - f(y)| = m + 2r$. 
    
%     If $f = \alpha g + \beta h$ where $g, h$ have lower rank than $f$, then $g$ must have a slope bound of $\frac m \alpha$ and $h$ must have a slope bound of $\frac m \beta$. By the inductive hypothesis, 
%     \[f(x) - f(y) = \alpha(g(x) - g(y)) + \beta(h(x) - h(y))\]
%     \[\leq \alpha\left(\frac m \alpha + 2(r-1)\right) + \beta\left(\frac m \beta + 2(r-1)\right)\]
%     \[\leq 2m.\]

%     If $f = \max(g, h)$ where $g$ and $h$ are of lower rank than $f$, then $f$ has as a slope bound the maximum of the slope bounds of $g$ and $h$ and the result follows.
% \end{proof}

% \subsection{Upper Bound on Change to IP Solution}

% Blair and Jeroslow's construction shows that there is a Gomory function whose value gives the optimal value of (\ref{eqn:IP}). Our next task is to follow their construction to give a slope bound and rank bound for this function in our case. See sections 4 and 5 of \cite{blair1982ip}. Let $P = |\pbasis(T)|$ be the size of the polymer basis (the number of variables in the IP), and let $S$ be the maximum number of monomers in any polymer. Let $M$ be the number of monomer types.

% Their construction is inductive, and the function in question is at level $NK_3$ of this inductive construction. $N$ is essentially a bound on the denominators of elements in the objective function, so in our case $N = 1$ as our objective function has all coefficients equal to 1. This value $K_3$ is constructed from three other values as the expression $M_1M_3 + M_2$. These values can each be bounded, some based on another constant $K_2$ which will be bounded next:

% \begin{enumerate}
%     \item $M_1$ is essentially a bound on how quickly the objective value of the corresponding real-valued linear program can change as the right-hand side changes. The optimal value of a linear program is always one of some set of $\lambda_i \cdot v$ where the $\lambda_i$ come from the extreme points of a polyhedron; they bound $M_1$ by the maximum norm of these $\lambda_i$. A bound in our case is $P$; if there was a $\lambda_i$ whose elements summed to more than $P$, then this would imply we could get a configuration with more total polymers (as the sum of polymer counts is our objective function) than monomers, which is impossible. 
%     \item $M_2$ is the maximum value of the objective function when all variables are at most $K_2$, which in this case is $PK_2$. 
%     \item $M_3$ is the maximum norm of the constraint matrix times the vector of variables when all variables are at most $K_2$. In TBN language, this gives the number of monomers present in a configuration with $K_2$ copies of every polymer in the polymer basis. The elements of the constraint matrix are bounded by $S$, so $M_3$ is bounded by $SPK_2$.
% \end{enumerate}

% Thus, $K_3 = M_1M_3 + M_2 \leq SP^2K_2$. In the paper, the value of $K_2$ is constructed by taking subsets of variables such that the space of $x$ such that $\sum a_jx_j = 0$ is one-dimensional. In TBN language, this corresponds to considering subsets of polymer types such that there is exactly one way (up to multiplication by a constant) to take a configuration of some of those polymer types, and reconfigure it into the rest of those polymer types. The value $K_2$ is as large as the greatest number of a single polymer type that may be necessary for such a reconfiguration.

% \todoi{Find and cite a source on the maximum element of a matrix inverse}
% To bound this, we first observe that no such subset can have more than $M$ elements; if it did, then the space of solutions, as the set of solutions to a system of homogeneous linear equations with more variables than equations, would be more than one-dimensional. It follows that we can find the solutions to this homogeneous system of equations by inverting an $M \times M$ matrix whose elements are bounded by $S$. The elements of this inverse are bounded by $2^MS$, so this is also a bound on our constant $K_2$. 

% Thus, $K_3 \leq S^2P^22^M$. 





% We now use a construction similar to their corollary 5.10 to show the following:

% \begin{lem}
%     \label{lem:gomory_variable_values}
%     Suppose $(x_i^*)$ is an optimal solution to (\ref{eqn:IP}). Let $M$ be the vector of the right-hand side of the equalities, and let $M'$ be some alternate right-hand side. Then there exist Gomory functions $\{g_p : p \in \pbasis(T)\}$ (which may depend on $M'$) such that:
%     \begin{enumerate}
%         \item $g_p(M) = x_p^*, \forall p \in \pbasis(T)$
%         \item Each $g_p$ has rank at most ZYX and slope bound YZX.
%     \end{enumerate}
% \end{lem}

% \begin{proof}
%     Our strategy is to construct integer programs that find the value for each $x_i$ that is as close as possible to $x_i^*$ while still being an optimal solution for the new right-hand side. These IPs then must have optimal values that are described by Gomory functions as the right-hand side changes.
%     Let $g$ be the Gomory function whose value gives the optimal value of (\ref{eqn:IP}). Let $\alpha_0$ be the optimal value of that IP. Define the following two IP problems. First,
%     \begin{equation}
%         \label{eqn:IP_value_max}
%         \begin{split}
%         \text{max}& \quad &&x_1 \\
%         \text{s.t.}& \quad &&\sum_{p \in \mathcal P(T)} p(M) x_p = T(M) \quad &&&\forall M \in m(T) \\
%         & \quad &&\sum_{p \in \mathcal P(T)} x_p = \alpha_0 \\
%         & \quad x_1 \leq x_1^*\\
%         &&x_p \geq 0 \quad &&&\forall p \in \mathcal P(T)
%         \end{split}
%     \end{equation}
%     Second, 
%     \begin{equation}
%         \label{eqn:IP_value_min}
%         \begin{split}
%         \text{min}& \quad &&x_1 \\
%         \text{s.t.}& \quad &&\sum_{p \in \mathcal P(T)} p(M) x_p = T(M) \quad &&&\forall M \in m(T) \\
%         & \quad &&\sum_{p \in \mathcal P(T)} x_p = \alpha_0 \\
%         & \quad x_1 \geq x_1^*\\
%         &&x_p \geq 0 \quad &&&\forall p \in \mathcal P(T)
%         \end{split}
%     \end{equation}

%     The values of these two IPs give, respectively, the largest and smallest possible values of $x_1$ in an optimal solution to (\ref{eqn:IP}). Let $g_{max}$ and $g_{min}$ be the value functions of these integer programs; they are Gomory functions, and their value on the right-hand side given here must equal $x_1^*$. \todoi{I think constants are not actually Gomory functions so some work may be needed here that it's okay to include the constant $x_1^*$ in this definition. For now I'm going to write it as though this is a Gomory function. Alternatively, as I have now done, throw in an extra constraint to the above IPs requiring $x_1$ greater or less than $x_1^*$ and then argue that it's fine to have an inequality in the IP}
%     For each of these two functions, we can then describe two new IPs describing the value of $x_2$, one maximizing it and one minimizing it, both of which have optimal value equal to $x_2^*$ and both of which have value functions given by a Gomory function. We can continue this process for all variables sequentially. 
%     Recall that the original IP problem describes stable configurations of a TBN whose monomer counts are given by the right-hand side. We know that when we change the right-hand side, the IP must remain feasible, because there is still some stable configuration. It follows that if we change the right-hand side for these new IP problems, at each step, at least one of the two IP problems must be feasible; at the first step, there is some stable configuration of the new TBN, and it has either less or more (or the same) amount of polymer $p_1$. If it has less, then the first IP is feasible; if more, then the second is feasible. Choose a feasible problem and define $g_1$ to be its value function. Do this similarly for the other variables sequentially: construct two IPs with constraints that the values of all previous variables are set, either maximizing or minimizing the value of the current variable while constraining it to be at most or at least its value in the known optimal solution.
%     Each $g_p$ by definition has $g_p^*(M) = x_p^*$. And since they describe value functions that are feasible for the new right-hand side $M'$, they are also defined there. \todoi{add an argument about the slope bound of these functions.}
    
% \end{proof}
% We are now ready to prove the main result of this section.

% \begin{proof}[Proof of \cref{thm:upperlimit}]
%     Let $\alpha$ be a configuration of $T$; we will find a configuration of $T'$ that is close to $\alpha$. The same argument works starting from a configuration of $T'$ to find a configuration in $T$.
    
%     By \cref{lem:gomory_variable_values}, for each polymer type in $\pbasis(T)$, there is a Gomory function with slope bound XYZ and rank ZYX whose value on the vector of monomer counts of $T$ and $T'$ respectively give the count of that polymer in $\alpha$ and in some stable configuration $\beta$ of $T'$. By \cref{lem:slopebound}, the value of this function for each polymer differs by at most $XYZ + 2ZYX$. Thus, as each polymer count could differ by this much, the total distance between the configurations is bounded by this amount times the size of the polymer basis, giving a final bound of BOUND\_GOES\_HERE.
% \end{proof}
